SAFE^d: Self-Attestation For Networks of Heterogeneous Embedded Devices

The Internet of Things (IoT) is an emerging paradigm that allows to set large networks of small and independent devices. To ensure their integrity, practitioners employ so-called Remote Attestation (RA) schemes. Classic RA schemes require a central and powerful entity, called Verifier, that has mainly two duties: (i) it manages the entire process of attestation, and (ii) it contains all the proofs for validating the devices' integrity. However, having a central Verifier makes the network dependent upon an external entity and introduces a single point of failure for security. In this work, we propose SAFE^d: the first RA schema that allows a pair of IoT devices to validate their integrity without relying on an external Verifier. Our approach overcomes previous limitations by spreading the proofs among multiple IoT devices and using novel cryptographic mechanisms to ensure secure communications. Moreover, the entire IoT network can collaboratively isolate tampered devices and recover missing proofs in case of anomalies. We evaluate our schema through an implementation for Raspberry Pi platform and a network simulation. The results show that SAFE^d can detect infected devices and recover up to 99.9% of proofs in case of faults or attacks. Moreover, we managed to protect up to 10K devices with a logarithmic overhead on the network and on the devices' memory.

==> dump.tex <==


\section{Preliminaries}
- Network of many heterogeneous devices with either static or dynamic topology
- Network can be either static or dynamic with no further assumption
- Devices that do not answer to query are either considered as dead or compromised, depending on the kind on query
- ...

\begin{acks}
We thank the Information System Technology Design (ISTD) department at the Singapore University of Technology and Design (SUTD) for taking part to this project.
\end{acks}

\subsection{old remote attestation background}

\todo{@AV: this is good for thesis}

The most interesting proposal so far regards remote attestation, a protocol for detecting malware presence on embedded systems, in which a remote part (Verifier) verifies software integrity of another one (Prover) by checking the latter's state. This usually means for the Prover to sign critical memory regions in an authenticated token and send the result to the Verifier for approval \cite{minimalist-attestation}. Different approaches have been explored to date: \textit{software-based} attestation requires no secure hardware but has unrealistic assumptions for practical implementations (passive attacker during attestation, tight time constraints) \cite{software-based}; \textit{hardware-based} attestation offers improved security guarantees by means of a trusted hardware but it is more suitable for general-purpose platforms since it is often too complex and expensive for low-end embedded devices; \textit{hybrid-based} attestation is a middle ground that tries to minimize hardware security features required for enabling secure remote attestation \cite{smart,trustlite,tytan}. The efficacy of hybrid approaches have been demonstrated in the single prover scenario thanks to the minimalistic features it requires: using just a Read Only Memory (ROM) and a Memory Protection Unit (MPU) it is able to guarantee atomicity of operations, memory isolation and exclusive access to secret keys. Even though the practice of single-prover attestation is well-established, in order to be effective in a multi-prover context, additional issues should be taken into account: discovery of - possibly dynamic - topologies, key management, routing, device heterogeneity.


==> evaluation_old.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate different metrics of $\text{SAFE}^d$.
First, we measure the 
network overhead (Section~\ref{ssec:performance}) and
memory footprint (Section~\ref{ssec:memory-footprint}).
Then, we measure how the \emph{proofs} get distributed among the devices 
(Section~\ref{ssec:load-spreading}) and the resilience of the network in the 
presence of attacks (Section~\ref{ssec:resilience}).
Finally, we discuss $\text{SAFE}^d$ security properties 
(Section~\ref{ssec:securityconsideration}).

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{img/messages.png}
		\caption{Number of messages per second.}
		\label{fig:messages}
    \end{subfigure}
    \hfill
	\begin{subfigure}[t]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/ftable.png}
		\caption{Average finger table size.}
		\label{fig:fingertablesize}
	\end{subfigure}
    \hfill
	\begin{subfigure}[t]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/resilience.png}
		\caption{Resilience.}
		\label{fig:resilience}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/percentage.png}
		\caption{Random source distribution.}
		\label{fig:random}
	\end{subfigure}
	\caption{Network overhead, finger table size, resilience measurements and 
	\emph{proofs} distribution of $\text{SAFE}^d$ prototype.}
	\label{fig:three graphs}
\end{figure}

\paragraph*{\textbf{Network Settings}}
Before we describe the experiments and the relative results
we illustrate the networks settings used for our experiments.
\begin{itemize}
	\item \textbf{Raspberry Pi}: we mounted a small network of Raspberry~Pi~3 
	composed by $4$ devices.
	This setting was used to measure the performances of $\text{SAFE}^d$ with different
	combination of \emph{overlays} and a fixed number of devices.
	Moreover, the Raspberry Pis was useful to prove the protocol claims on real 
	devices.
	\item \textbf{Omnet++}: we used Omnet++ to simulate a network of IoT 
	devices that contained up to $10$k entities.
	We used this setting to stress the performances of $\text{SAFE}^d$ 
	in presence of thousand devices and with different combinations 
	\emph{overlays}.
\end{itemize}
%	\item \textbf{Docker}\todo{update it}: we mounted a virtual network 
%	composed by various number
%	of Docker containers (from $10$ to $50$), each of them representing a 
%device.
%	We used this setting to measure the performances of $\text{SAFE}^d$ with 
%larger number of devices and a fixed number of \emph{overlays}.
%\end{itemize}


\subsection{Network Overhead}
\label{ssec:performance}

We measure the network overhead introduced by $\text{SAFE}^d$ in terms of global messages exchanged and messages process time.

\paragraph*{\textbf{Global Messages Exchanged.}} 
Figure~\ref{fig:messages} shows the average number of messages exchanged
per second (\ie msg/sec) with different network settings.
In our implementation, we handle two types of message:
\begin{itemize}
	\item \textbf{Certification messages}: they are used only during the certification
	phase (Section~\ref{ssec:certification-phase}) and 
	require $256 \times o$ bytes, where $o$ is the number of \emph{overlays} (\eg $1$KB for $4$ \emph{overlays}).
	These messages are more expensive in terms of size but they are only used during the \emph{Certification Phase}.
	\item \textbf{Routine messages}: the other messages exchanged in our prototype have a fixed size of $384$ bytes plus $68 \times s$ bytes, where $s$ is the successor list size (\eg $520$B with $2$ successors).
	They compose the vast majority of the network communication.
	Furthermore, $s$ is a fixed parameter of the network, thus the message size remains constant throughout the execution.
\end{itemize}
We measured the messages exchanged by tuning two properties.
We varied the number of \emph{overlays} from $2$ to $8$ on the Raspberry Pi 
network (dotted line),
while we varied the number of devices from $10$ to $50$ on the Docker
network (solid line).
The results from the Raspberry Pi network show a linear 
growth of the number of messages with the increase of the \emph{overlays}.
We measured around $2.5$ msg/sec by using $4$ devices and $2$ \emph{overlays},
till reaching around $9$ msg/sec by using $4$ devices an $8$ \emph{overlays}.
This result is intuitive because each \emph{overlay} works independently, and therefore,
they require a separate set of messages for their operations.
A different behavior is, instead, observed for the Docker network, that shows a
logarithmic growth of the number of messages with the increase of the devices.
In this case, we measured up to $2$msg/sec on average with $50$ devices and a
single \emph{overlay}.
This pattern is a consequence of Chord algorithm, which scales well in terms of network size.

To sum up, the network overhead introduced by $\text{SAFE}^d$ scales logarithmically with the number of devices.
Previous works~\cite{us-aid,pasta} do not propose an analysis for the network overhead.
However, the security of their communication channels relies on the prior execution of a key exchange protocol between each pair of devices that needs to exchange data.
Considering that a device needs to communicate with every neighbour, we can infer that the overall complexity for the network is at least quadratic on the average number of neighbour a device has inside the network.

\paragraph*{\textbf{Message Time Elapsed}}
We measure the time required to process a single message in a Raspberry Pi.
We did not considered the \emph{Certification} messages phase because 
they are used only during the initial part of the protocol.
We also ignored Docker containers performances because
we focus on real device scenarios.
As a result, any message required on average $9.1$ms (with a standard deviation of
$6.3$) to be processed without using cryptography,
while around the double, $18$ms (with a standard deviation of $9.2$), using the
cryptography described in Section~\ref{ssec:secure-device-comm}.
As already observed in~\cite{us-aid,pasta}, the cryptography is the predominant part during the protocol execution.

\subsection{Memory Footprint}
\label{ssec:memory-footprint}

Each device uses $64$, $1218$, $294$ and $256$ bytes respectively for the UID, the private RSA key, the public RSA key and the certificate.
For each overlay, it uses $32$ bytes for the secret, $68$ bytes for its own OID and its predecessor OID, $68$ bytes for each entry in the successor list, $68$ bytes for the entries in the finger list and $128$ bytes for each element inside the proof storage.
The overall memory usage $M$, expressed in bytes, can be computed as follows:
\begin{equation*}
\begin{split}
M = 1832+[168+68\times{s}+68\times{f}+128\times{p}]\times{o},
\end{split}
\end{equation*}
where $s$ is the size of the successor list, 
$f$ is the size of the finger table, $p$ is the number of \emph{proofs} and $o$ the number of \emph{overlays}. The size of the successor list $s$ is a fixed parameter that remains constant during the protocol execution.
The finger list size $f$, instead, has an upper bound of $\log(n)$, with $n$ the total number of devices inside the network.
In Figure~\ref{fig:fingertablesize}, we support the previous claim analyzing the finger table size in both
Raspberry Pi (dashed line) and Docker (solid line) networks.
This table is used by Chord to optimize packets routing (see Section~\ref{ssec:chord}).
Each \emph{overlay} maintains a separate table, and their entries represent other devices in the same \emph{overlay}.
Similarly to the global message exchanged, we observe two patterns.
For the Raspberry Pi network, the finger table grows linearly.
It ranges from around $0.3$KB, for $4$ devices 
and $2$ \emph{overlays}, to around $1.2$KB, for $4$ devices and $8$ overlays.
This pattern is linear because each device maintains a separate table for each
\emph{overlay}.
On the other hand, the Docker network's size grows logarithmically
reaching up to $0.3$KB, for $50$ devices and a single \emph{overlay}.
This is because the finger table by design contains at most a logarithmic number of entries with respect to the network size.

To sum up, the space required for each device till now is scalable because it requires an
amount of memory which is logarithmic with the number of devices.
In the next paragraph, we will discuss the number of proofs $p$ that a device is expected to store.

\subsection{Proofs Spreading}
\label{ssec:load-spreading}


We analyze the \emph{proofs} distribution in a network from two perspectives:
at first, we discuss the \emph{proofs} distribution in presence of a single \emph{overlay};
then, we analyze the case with smaller networks and multiple \emph{overlays}.

Figure~\ref{fig:random} shows an analysis of the \emph{proofs} distribution in a single \emph{overlay}.
To calculate the distribution, we considered the distances between each pair of consecutive \emph{proofs}.
The \emph{normalized distance} is shown in the y-axis of the plot, while the x-axis shows the number of \emph{proofs} present inside the \emph{overlay}.
To give a comprehensive view, we propose four different curves:
\begin{enumerate*}[label=(\roman*)]
	\item the \emph{ideal} distance as a thin-dashed line,
	\item the \emph{minimum} distance as a dot-dashed line,
	\item the \emph{average} distance as a solid line, and
	\item the \emph{maximum} distance as a bold-dashed line.
\end{enumerate*}
We observe that the average \emph{normalized distance} remains close to the ideal case, while the maximum \emph{normalized distance} converges towards it. At $50$ \emph{proofs}, the \emph{overlay} reaches an average distance of $5\%$ with a maximum distance of $10\%$.
The trend shows that a more crowded \emph{overlay} brings to a more uniform distribution of \emph{proofs}.
This is due to the location of both devices and \emph{proofs} that is regulated by random identifier, \ie OIDs and UIDs.
In fact, a random process is supposed to generate a roughly uniform distribution after enough extractions, that we empirically estimated being around $50$ \emph{proofs}.

Having independent and random \emph{proofs} helps obtaining a uniform distribution for smaller networks (\eg $10$ devices) by tuning the number of \emph{overlays}.
Each \emph{overlay} is indeed completely independent from the others.
Thus, we can consider the nodes that populate a particular \emph{overlay} as separate entities from the others.
This means that, in case of networks with $10$ devices, we can balance the distribution of the \emph{proofs} by setting $5$ \emph{overlays}.
In this way, we reach a population of $50$ independent entities. 

To sum up, the number of proofs $p$ that a device stores is bounded and can be forced to reach the ideal value (\ie $1$ \emph{proofs} for each \emph{overlay}) even in small networks.
Considering the overall memory consumption, $\text{SAFE}^d$ is a clear improvement with respect to previous works that are either an order of magnitude more expensive~\cite{pasta} or have a quadratic dependence on unpredictable parameters~\cite{us-aid}.

\subsection{Resilience}
\label{ssec:resilience}

The purpose of this experiment is to measure the ability of $\text{SAFE}^d$ of recovering
missing \emph{proofs} in case of attacks or faults.
We performed this measurement using the Raspberry Pi network.
Furthermore, we modeled a powerful attacker that 
randomly destroys all the \emph{proofs} of a device.
This attack is tuned by a drop rate which indicates the probability 
of a device to erase its own \emph{proofs} on all \emph{overlays}.
For instance, a drop rate of $5\%$ means that each device will randomly erase its 
own \emph{proofs} during $5$ operations out of $100$ on average.
We tested different combination of drop rate and number of
\emph{overlays} to observe the different responses.

Figure~\ref{fig:resilience} shows the results of our experiments.
We varied the drop rate from $5\%$ to $30\%$, 
which means that in the worst case each 
device removed all of its own \emph{proofs} one out of three operations.
The \emph{overlays}, instead, ranged from $2$ to $8$.
The y-axis shows the \emph{resilience index}, 
which is the ratio between the number of \emph{proofs}
correctly recovered and the number of non-retrieved \emph{proofs}.
According to the attestation algorithm (Section~\ref{ssec:attestation}), in case of non-retrieved \emph{proofs}, the \emph{Verifier} attempts to recover the
missing information from the other \emph{overlays}.
Therefore, the \emph{resilience index} tends to $100$ if all the \emph{proofs}
were correctly recovered, otherwise it goes to $0$.
The plot shows that with the increases of the \emph{overlays}, the \emph{resilience index} tends to reach $100$ even in presence of an high drop rate.
More precisely, we manage to recover $99.7\%$ of the \emph{proofs} with $8$ \emph{overlays}.
Overall, the \emph{resilience index} stays above $97.2\%$ by using only $4$ \emph{overlays} with a drop rate of $20\%$.

This experiment shows that the \emph{overlays} can be effectively used to recover
the network in the presence of attacks, even though the network is small.
 

\subsection{Security Consideration}
\label{ssec:securityconsideration}
We describe how $\text{SAFE}^d$ reacts against different attacker scenarios.

\paragraph*{\textbf{Tampered Devices}}
An attacker may infect a device and take control of it.
Since we use a trusted anchor, we consider the \emph{secure world} 
as protected, while the \emph{normal world} can be under attacker control.
Therefore, $\text{SAFE}^d$ protocol is protected by design.
Moreover, all the packets that transit through the \emph{normal world} are encrypted, 
thus outside the attacker range.
However, an attacker may avoid invoking trusted anchor code by compromising
\emph{normal world} scheduler. We mitigate this problem by adopting a blind 
scheduling (Section~\ref{sec:implementation}) that 
avoids an attacker to disable a specific $\text{SAFE}^d$ operation 
(\eg attestation) without stopping the entire device, thus being detected.

To test $\text{SAFE}^d$ effectiveness, we verified that the other devices are able to spot the modified code inside the \emph{normal world}.

\paragraph*{\textbf{Attacks against the Network}}
All the messages exchanged among trusted anchors are encrypted
(Section~\ref{ssec:secure-device-comm})
and only devices that joined the network can communicate among each other
(Section~\ref{ssec:certification-phase}).
Man-in-the-middle~\cite{asokan2003man} attacks are mitigated by design:
\begin{enumerate*}[label=(\roman*)]
	\item the body is protected by the symmetric key $K_{AB}$,
	\item the header can be manipulated only by the trusted anchors of
	authorized devices.
\end{enumerate*}
We also include nonces to avoid replay attacks.
This enhances robustness even in case of corrupted devices as long as 
their trusted anchor remains intact.

\paragraph*{\textbf{Physical attacks}}
According to DARPA attacker model~\cite{darpa}, a device which receives
a physical attack is temporarily removed from the network.
Previous authors~\cite{darpa,scapi,pasta} proposed to use a heartbeat to keep the devices
synchronized. In this way, a device that goes temporarily off-line cannot get
aligned with the heartbeat, and therefore, enabling the detection of the attack.
However, establishing a heartbeat protocol implies the presence of loosely synchronized and secure clocks in every device. $\text{SAFE}^d$ overcomes this requirement by using the communication timeouts and nonces to detect network disconnections.
During the protocol execution, each device periodically contacts its successor to assess its status.
In case a timeout occurs, the device uses the successor list to contact the closest node following the old one.
The contacted device will further check if its predecessor left the network, and if so, it will acquire the message sender as new predecessor, while launching an alert for a possible physical attack.
The double check adds robustness against simple network malfunctions.
To enhance the protection against physical attacks, we further propose a certificate revocation strategy that will be discussed in Section~\ref{sec:discussion}.

\paragraph*{\textbf{Denial-of-Service}} 
We do not protect against denial-of-service in case of an entire compromised 
network (\eg all the messages are dropped). 
However, we can recover partial information loss by combining multiple \emph{overlays}
and our attestation protocol (Section~\ref{ssec:resilience}).

==> introduction_backup.tex <==
\section{Introduction}

\subsection{Overview}
In the last decade we have been witnessing the rise of a completely new way of computing 
and collecting data, defined as the Internet of Things (IoT). The most powerful concept 
bounded with the IoT world is the idea of a decentralized network, accessible remotely 
through the Internet and composed by heterogeneous devices, equipped with a particular 
mixture of sensors, actuators and processors. The strength of this approach resides in the adaptability of the network itself, with the range of applications going from industrial control systems to small home-appliances, making it suitable for virtually all context in everyday life. The forecasts on the IoT market for the next years just confirm this wide adoption, showing that the new paradigm is expected to reach a worth-value of \$1.2 trillions in 2022 \cite{iot-stats1}, with the number of IoT-related connections touching 18 billions \cite{iot-stats2}. However, as usual, not all that glitters is gold: IoT devices are often constrained systems without a proper security design and are called to handle sensitive information and safety-critical tasks. The result of this unstable setting has been already shown with the Mirai botnet \cite{mirai}, composed largely by infected embedded devices, that took the Internet by storm in late 2016 when it attacked several high-profile targets with huge distributed denial-of-service attacks. Given the decentralized nature and the low computing power at disposal, classical security measures are not applicable in this context; it is then clear the urge for novel ways of securing such environments. With this paper we want to further investigate remote attestation as a solution for securing such environments. In particular, we want to propose a completely new approach to remotely verify the integrity of a swarm of IoT devices. The papers proposed so far assume an unique, trusted Verifier that is aware of the cardinality of the network and correctly executes attestation quests. This assumption forces a spanning tree strategy, with the Verifier as root of a tree in which the network nodes recursively propagate requests and aggregate results. The spanning tree approach unavoidably introduces a single-point of failure, impersonated by the Verifier, through which a potential attacker can bring down the protocol. Moreover, the aggregation process introduces severe overhead to the limited IoT devices.

\paragraph{Objectives}
The solution must be scalable with respect to the number of devices and must provide unforgeability and freshness of verification in order to detect and identify compromised devices. It must be agnostic with respect to the type of devices in the network and resilient to failures. Given the limited environment, the protocol must have both low computational complexity and small memory fingerprint. As an additional feature, the protocol should try to limit Denial-of-Service (DoS) attacks.

\paragraph{Contributions}
 In this paper we propose the first multi-verifier approach in which every device can at the same time assume both the guise of Prover and Verifier. To reach this objective we reviewed and added new functionalities to the Chord protocol, on top of which we then built our multi-verifier scheme. Finally we deployed an evaluation prototype and carried out a performance analysis through both a virtual environment and a real network of Raspberry PIs to prove the quality of our solution.

\paragraph{Outline}
In section 2 we describe previous works on this subject. In section 3 we introduce the background concepts related to our paper. In section 4 we describe our proposal for a highly distributed remote attestation of IoT networks. In section 5 we show the experimental results. In section 6 we further discuss the implication of the results.

==> relatedwork_backup.tex <==
\section{Related Work}
\label{sec:related-work}

\todo{to shrink, troppo brodo e poco delta con HiDRA}
The more recent literature has dealt with the underlined problems and proposed several solutions for implementing a practical collective attestation, also called swarm attestation. A common idea behind these protocols is the arrangement of the network's nodes in a spanning tree rooted at the Verifier. Once an attestation request is sent down the tree, every node is in charge of forwarding it to its children nodes and of aggregating the responses, thus reaching a logarithmic complexity by dividing the burden of propagation and elaboration across all the devices. SEDA \cite{seda} has been the first step toward a practical swarm attestation. In it, the Verifier chooses a random device as initiator and sends an attestation request to it. Every device accepts the request's sender as its parent and forwards it to its neighbors. Once the parent receive all of its children's reports, it aggregates them into a single report and send it back. The process continues recursively until the initiator receives all reports and combines them, signing the result using its private key and returning it to the verifier. Despite the good performances and the minimal hardware assumptions made, SEDA presents several unresolved issues: it is not clear how the Verifier manages timeouts on the responses; the final report includes only the number of devices that passed attestation; a tampered node in the spanning tree may compromise the report of all the sub-tree rooted on it; the tree must be static during attestation process; the protocol requires trust in all intermediaries. Trying to overcome these limitations, SANA \cite{sana} enhances SEDA by providing a new scheme based upon Optimistic Aggregate Signatures for a more efficient aggregation of reports. To limit the need for trusted hardware, only targeted nodes are required to implement attestation and all aggregators can be untrusted; with this renewed setup, a compromised node can at most tamper its own report. The major problem in this solution regards the possible severe overhead introduced by the OAS computation in both provers and aggregators. Another scheme proposed in order to bring SEDA closer to practice is \cite{lisa}: two different protocols that differ in the synchronicity of the request's replies. In Lisa-\textalpha nodes act independently and asynchronously, relying in each other just for forwarding requests and replying responses; in Lisa-s, instead, each nodes must wait for all its children to respond before replying to its parent. The first variant has high communication overhead and imposes all the burden of verification on the Verifier. The second one addresses these problems but requires all nodes in the forwarding-path to be awake until process completion. DARPA \cite{darpa} builds on top of previous works and uses absence detection for dealing with a stronger attacker capable of physical tampering. The idea behind DARPA is that an adversary that physically tampers a node needs a certain amount of time to physically access that device. Hence each neighbour can detect an absence by periodically emitting the so-called heartbeat at regular time intervals and registering the responses. The Verifier can then detect any anomaly when collecting all the transactions. Relying on the underlying protocol for executing attestation, DARPA inevitably inherits all the limitations bounded with it. Moreover, the amount of heartbeat exchanged scales quadratically with the number of devices and a single missing heartbeat due to connection failures can cause a false positive alarm. SCAPI \cite{scapi} handles shortcomings of DARPA by reducing communication complexity, precisely identifying compromised devices and supporting highly dinamic and partioned network topologies. It introduces a better way to detect physical attacks where all nodes in the network share two common session keys that are periodically updated by a leader. A periodic update of the group secrets excludes offline devices, not letting them to team up once they are online again. The election of a leader for a group of nodes introduces additional complexity in the system; also, SCAPI relies on the strong assumption of a network with at least half of the nodes healthy and needs a storage size linear with the total number of devices.
